Wheeling: A diagrammatic analogue of the Duflo isomorphism

We construct and prove a diagrammatic version of the Duflo isomorphism between the invariant subalgebra of the symmetric algebra of a Lie algebra and the center of the universal enveloping algebra. This version implies the original for metrized Lie algebras (Lie algebras with an invariant non-degenerate bilinear form). As an application of this isomorphism, we will compute the Kontsevich integral of the unknot and the Hopf link to all orders. At the core of the proof, we use an elementary property of the Hopf link which can be summarized by the equation ``1+1=2'' in abacus arithmetic: doubling one component of the Hopf link is equivalent to taking the connected sum of two Hopf links. This property of the Hopf link turns out, when suitably interpreted, to be exactly the property required for the Duflo map to be multiplicative. To compute the Kontsevich integral of the unknot, we use a property of the unknot that can be summarized by ``n * 0 = 0'': the n-fold connected cabling of the unknot is again an unknot.

==> Makefile <==
name=thesis
texinputs=macros.tex defs.tex intro.tex liealg.tex vassiliev.tex \
	 kontsevich.tex wheeling.tex wheels.tex cyclic.tex coefficients.tex \
	 main.tex main.bbl main.blg ucthesis.cls uct10.clo
inputs = $(texinputs) dptsymb.mf dptsymb.sty Makefile

# I need this to run reasonably under emacs.
#TEX = latex --interaction nonstopmode
TEX = latex

all: $(name).dvi

draws: draws.trans
	touch main.aux

Makefile.trans: figs.list;
	xargs transfig -M Makefile.trans.tmp -L pstex < figs.list
	sed -e "s/^all/draws.trans/" -e "s/Makefile.trans.tmp/Makefile.trans/g" \
		 < Makefile.trans.tmp > Makefile.trans
	rm Makefile.trans.tmp

include Makefile.trans

# Run all from Makefile.trans.  This is suboptimal...
# draws: all

$(name).dvi: main.dvi;
	cp -p main.dvi $(name).dvi

main.dvi: main.tex $(texinputs) Makefile.trans main.aux
	mv figs.list figs.old
	cp -p main.aux main.aux-old
	$(TEX) main
	if cmp -s figs.list figs.old; then \
	  mv figs.old figs.list; \
	fi
	if cmp -s main.aux main.aux-old; then\
	  mv main.aux-old main.aux; \
	fi

main.bbl: knots.bib main.aux
	-bibtex main

bib:
	bibtex main

ps:     $(name).dvi;
	dvips $(name).dvi -o $(name).ps

$(name).ps:     $(name).dvi draws/*.eps
	dvips $(name).dvi -o $(name).ps

source.uu: main.tex $(inputs) draws/*.fig makefile main.hdr $(name).hdr\
		recycling;
	tar cvf main.tar main.tex $(inputs) makefile $(name).hdr\
		main.hdr draws/*.fig recycling
	ls -l main.tar
	gzip -9 -f main.tar
	rm -f source.uu
	cat main.hdr > source.uu
	echo "# $(name): Packed on "`date`" by "`whoami`" on "`hostname` \
		>> source.uu
	echo "" >> source.uu
	uuencode main.tar.gz main.tar.gz >> source.uu
	ls -l source.uu
	rm -f main.tar.gz

source.tar.gz: main.tex $(inputs) draws/*.fig Makefile recycling
	tar hcvf source.tar $^
	ls -l source.tar
	gzip -9 -f source.tar

$(name).tar.gz: main.tex $(inputs) Makefile
#	sed sX\\\\todayX`date +"%h.~%d,~19%y"`X main.tex > $(name).tex
	tar hcvf $(name).tar $(inputs) draws/*.tex draws/*.eps
#	ls -l $(name).tar
	gzip -9 -f $(name).tar

info:	;
	ls -tl main.tex $(inputs) draws/*.fig makefile main.hdr $(name).hdr \
		recycling | head
	if [ -f source.uu ]; then grep Packed source.uu; \
		else echo "no source.uu"; fi
	if [ -f main.uu ]; then grep Packed main.uu; \
		else echo "no main.uu"; fi
	if [ -f $(name).uu ]; then grep Packed $(name).uu; \
		else echo "no $(name).uu"; fi

figs.list:
	touch figs.list

main.aux:
	touch main.aux

#figs.list: figs.old
#	cp -p figs.old figs.list

# Makefile.trans cleans up the draws
clean::
	-rm *~ *.aux *.log *.dvi *.ps *.dvi.gz *.ps.gz *.bbl *.blg figs.list \
		draws/*.tex draws/*.eps draws/*.fig.bak *.uu *.toc transfig.tex



==> draws/1n-twist.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/1n-twist.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1394,946)(879,-1975)
\end{picture}


==> draws/2wheel.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/2wheel.eps}%
\end{picture}%
\setlength{\unitlength}{1973sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1224,614)(889,-368)
\end{picture}


==> draws/4wheel.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/4wheel.eps}%
\end{picture}%
\setlength{\unitlength}{1973sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(924,924)(3739,-523)
\end{picture}


==> draws/6wheel.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/6wheel.eps}%
\end{picture}%
\setlength{\unitlength}{1973sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1074,1074)(1864,-1198)
\end{picture}


==> draws/A-examp.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/A-examp.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4428,1217)(2699,-1727)
\end{picture}


==> draws/AS-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/AS-1.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3572,2095)(906,-2054)
\end{picture}


==> draws/AS-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/AS-2.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3534,1935)(612,-5119)
\end{picture}


==> draws/AS-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/AS-3.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3227,1925)(919,-5121)
\end{picture}


==> draws/AS-diag-0.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/AS-diag-0.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3329,1927)(834,-5116)
\end{picture}


==> draws/AS-diag-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/AS-diag-1.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3239,1927)(924,-5116)
\end{picture}


==> draws/AS-diag-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/AS-diag-2.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3239,1927)(924,-5116)
\end{picture}


==> draws/B-examp.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/B-examp.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2000,1824)(889,-1873)
\end{picture}


==> draws/DiagonalGluing.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/DiagonalGluing.eps}%
\end{picture}%
\setlength{\unitlength}{1973sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(695,624)(666,-523)
\end{picture}


==> draws/HopfSum.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/HopfSum.eps}%
\end{picture}%
\setlength{\unitlength}{1492sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4610,2601)(2354,-3548)
\end{picture}


==> draws/One.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/One.eps}%
\end{picture}%
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1916,2304)(1113,-2473)
\end{picture}


==> draws/OneOneTwo.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/OneOneTwo.eps}%
\end{picture}%
\setlength{\unitlength}{1367sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4692,2889)(2883,-3808)
\end{picture}


==> draws/SideGluing.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/SideGluing.eps}%
\end{picture}%
\setlength{\unitlength}{1973sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(695,624)(366,-223)
\end{picture}


==> draws/Zero.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/Zero.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3130,3130)(8129,-5485)
\end{picture}


==> draws/adx.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/adx.eps}%
\end{picture}%
\setlength{\unitlength}{2486sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(548,1374)(856,-1423)
\put(856,-826){\makebox(0,0)[rb]{\smash{\SetFigFont{10}{12.0}{\familydefault}{\mddefault}{\updefault}\special{ps: gsave 0 0 0 setrgbcolor}$x$\special{ps: grestore}}}}
\end{picture}


==> draws/cyclic-trivalent-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/cyclic-trivalent-2.eps}%
\end{picture}%
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1313,1126)(844,-1490)
\end{picture}


==> draws/cyclic-trivalent-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/cyclic-trivalent-3.eps}%
\end{picture}%
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1313,1111)(844,-1475)
\end{picture}


==> draws/double-lasso-chord.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/double-lasso-chord.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1423,2496)(1297,-2524)
\end{picture}


==> draws/double-twist.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/double-twist.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(787,2459)(2174,-2479)
\end{picture}


==> draws/figure8-closed.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/figure8-closed.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4236,5947)(1695,-6345)
\end{picture}


==> draws/figure8-open.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/figure8-open.eps}%
\end{picture}%
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1079,3759)(2154,-3823)
\end{picture}


==> draws/fulltwists.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/fulltwists.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4103,4751)(3324,-5006)
\end{picture}


==> draws/id2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/id2.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(403,3688)(1577,-4155)
\end{picture}


==> draws/jacobi-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-1.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3665,2262)(498,-5443)
\end{picture}


==> draws/jacobi-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-2.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3514,2254)(641,-5443)
\end{picture}


==> draws/jacobi-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-3.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3239,2254)(916,-5443)
\end{picture}


==> draws/jacobi-4.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-4.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3239,2254)(916,-5443)
\end{picture}


==> draws/jacobi-diag-0.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-diag-0.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3329,2033)(834,-5222)
\end{picture}


==> draws/jacobi-diag-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-diag-1.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3239,2033)(924,-5222)
\end{picture}


==> draws/jacobi-diag-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-diag-2.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3239,2033)(924,-5222)
\end{picture}


==> draws/jacobi-diag-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/jacobi-diag-3.eps}%
\end{picture}%
\setlength{\unitlength}{787sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3239,1927)(924,-5116)
\end{picture}


==> draws/line-circle-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/line-circle-1.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4414,2702)(2699,-2342)
\end{picture}


==> draws/line-circle-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/line-circle-2.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4498,2702)(2615,-2342)
\end{picture}


==> draws/line-circle-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/line-circle-3.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4175,2702)(2938,-2342)
\end{picture}


==> draws/line-circle-4.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/line-circle-4.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4100,2702)(3013,-2342)
\end{picture}


==> draws/line.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/line.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(66,2451)(2218,-2479)
\end{picture}


==> draws/matrix-trace.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/matrix-trace.eps}%
\end{picture}%
\setlength{\unitlength}{2486sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1047,1226)(1609,-1273)
\put(1846,-781){\makebox(0,0)[b]{\smash{\SetFigFont{9}{10.8}{\familydefault}{\mddefault}{\updefault}\special{ps: gsave 0 0 0 setrgbcolor}$M$\special{ps: grestore}}}}
\end{picture}


==> draws/metric-inv.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/metric-inv.eps}%
\end{picture}%
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1385,631)(576,-1569)
\end{picture}


==> draws/metric.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/metric.eps}%
\end{picture}%
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1385,631)(576,-1569)
\end{picture}


==> draws/n-twists.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/n-twists.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1394,2744)(879,-3773)
\end{picture}


==> draws/nCircus-diag-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/nCircus-diag-1.eps}%
\end{picture}%
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2746,2744)(878,-2559)
\end{picture}


==> draws/nCircus-diag-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/nCircus-diag-2.eps}%
\end{picture}%
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2746,2744)(878,-2739)
\end{picture}


==> draws/nCircus-examp.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/nCircus-examp.eps}%
\end{picture}%
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3203,2952)(662,-3247)
\end{picture}


==> draws/nZero.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/nZero.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3245,3364)(2275,-4016)
\end{picture}


==> draws/problem-integral.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/problem-integral.eps}%
\end{picture}%
\setlength{\unitlength}{99sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5438,5038)(882,-5480)
\end{picture}


==> draws/rloop-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/rloop-1.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2049,1509)(889,-973)
\end{picture}


==> draws/rloop-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/rloop-2.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2049,1509)(889,-973)
\end{picture}


==> draws/rloop-n.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/rloop-n.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2049,1509)(889,-973)
\end{picture}


==> draws/rloop.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/rloop.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2184,1509)(754,-973)
\end{picture}


==> draws/simple-crossing.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/simple-crossing.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3025,2816)(742,-2658)
\end{picture}


==> draws/simple-lasso.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/simple-lasso.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3719,2860)(391,-2736)
\end{picture}


==> draws/simple-single-lasso.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/simple-single-lasso.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(916,1236)(703,-2659)
\end{picture}


==> draws/simple-twist.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/simple-twist.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1502,1258)(892,-2671)
\end{picture}


==> draws/single-lasso-simp.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/single-lasso-simp.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(916,1236)(703,-2636)
\end{picture}


==> draws/single-lasso.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/single-lasso.eps}%
\end{picture}%
\setlength{\unitlength}{1243sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(916,1027)(893,-1868)
\put(901,-1051){\makebox(0,0)[rb]{\smash{\SetFigFont{5}{6.0}{\familydefault}{\mddefault}{\updefault}\special{ps: gsave 0 0 0 setrgbcolor}$L_1$\special{ps: grestore}}}}
\end{picture}


==> draws/sl2-glue-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/sl2-glue-1.eps}%
\end{picture}%
\setlength{\unitlength}{622sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1742,4454)(1380,-4268)
\end{picture}


==> draws/sl2-glue-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/sl2-glue-2.eps}%
\end{picture}%
\setlength{\unitlength}{622sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1742,4274)(1380,-4268)
\end{picture}


==> draws/sl2-glue-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/sl2-glue-3.eps}%
\end{picture}%
\setlength{\unitlength}{622sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2390,4274)(1380,-4268)
\end{picture}


==> draws/sl2-wheel-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/sl2-wheel-1.eps}%
\end{picture}%
\setlength{\unitlength}{497sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5340,2242)(481,-2828)
\end{picture}


==> draws/sl2-wheel-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/sl2-wheel-2.eps}%
\end{picture}%
\setlength{\unitlength}{497sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5340,2242)(481,-2828)
\end{picture}


==> draws/sl2-wheel-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/sl2-wheel-3.eps}%
\end{picture}%
\setlength{\unitlength}{497sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5340,2242)(481,-2828)
\end{picture}


==> draws/sl2-wheel-4.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/sl2-wheel-4.eps}%
\end{picture}%
\setlength{\unitlength}{497sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3180,1747)(481,-2333)
\end{picture}


==> draws/split-1.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/split-1.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3666,2894)(418,-2768)
\end{picture}


==> draws/split-2.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/split-2.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3666,2847)(418,-2768)
\end{picture}


==> draws/split-3.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/split-3.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3666,2907)(418,-2768)
\end{picture}


==> draws/split-4.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/split-4.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3666,2907)(418,-2768)
\end{picture}


==> draws/three-single-lassos.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/three-single-lassos.eps}%
\end{picture}%
\setlength{\unitlength}{829sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3360,2785)(571,-2691)
\put(3871,-736){\makebox(0,0)[lb]{\smash{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}\special{ps: gsave 0 0 0 setrgbcolor}-1\special{ps: grestore}}}}
\end{picture}


==> draws/trefoil-conn4cable.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/trefoil-conn4cable.eps}%
\end{picture}%
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5300,5065)(958,-5321)
\end{picture}


==> draws/trefoil-disconn4cable.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/trefoil-disconn4cable.eps}%
\end{picture}%
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5305,5066)(953,-5322)
\end{picture}


==> draws/trefoil-whitehead.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/trefoil-whitehead.eps}%
\end{picture}%
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5160,4870)(1030,-5229)
\end{picture}


==> draws/twist-lasso.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/twist-lasso.eps}%
\end{picture}%
\setlength{\unitlength}{1036sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1213,2474)(1748,-2494)
\end{picture}


==> draws/vertex-expand.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/vertex-expand.eps}%
\end{picture}%
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1400,1551)(1095,-2062)
\end{picture}


==> draws/vertex.tex <==
\begin{picture}(0,0)%
\includegraphics{draws/vertex.eps}%
\end{picture}%
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(1400,1551)(1095,-1942)
\end{picture}

